Parallel local search for solving Constraint Problems on the Cell Broadband Engine (Preliminary Results)

We explore the use of the Cell Broadband Engine (Cell/BE for short) for combinatorial optimization applications: we present a parallel version of a constraint-based local search algorithm that has been implemented on a multiprocessor BladeCenter machine with twin Cell/BE processors (total of 16 SPUs per blade). This algorithm was chosen because it fits very well the Cell/BE architecture and requires neither shared memory nor communication between processors, while retaining a compact memory footprint. We study the performance on several large optimization benchmarks and show that this achieves mostly linear time speedups, even sometimes super-linear. This is possible because the parallel implementation might explore simultaneously different parts of the search space and therefore converge faster towards the best sub-space and thus towards a solution. Besides getting speedups, the resulting times exhibit a much smaller variance, which benefits applications where a timely reply is critical.

==> table-data/all-interval-450.tex <==
 1 &      946.860 &    1.0 &     4661.870 &    1.0 \\
 2 &      470.421 &    2.0 &     1912.200 &    2.4 \\
 4 &      228.294 &    4.1 &      988.220 &    4.7 \\
 8 &      109.322 &    8.7 &      304.160 &   15.3 \\
12 &      102.831 &    9.2 &      443.550 &   10.5 \\
16 &       85.936 &   11.0 &      177.210 &   26.3 \\


==> table-data/all-interval-avg.tex <==
100 &        1.392 &    1.6 &    3.3 &    5.0 &    5.7 &    7.4 &        0.189 \\
150 &        9.496 &    2.3 &    4.4 &    6.3 &    9.0 &   10.4 &        0.910 \\
200 &       28.165 &    1.5 &    3.0 &    6.1 &    7.8 &    9.0 &        3.139 \\
250 &       61.437 &    1.8 &    3.8 &    5.1 &    6.5 &    9.8 &        6.282 \\
300 &      147.178 &    1.7 &    2.9 &    5.6 &    7.3 &    9.2 &       15.920 \\
350 &      346.790 &    2.3 &    4.4 &    5.6 &    9.6 &   12.2 &       28.359 \\
400 &      508.819 &    1.6 &    3.3 &    7.6 &    8.8 &   10.8 &       46.989 \\
450 &      946.860 &    2.0 &    4.1 &    8.7 &    9.2 &   11.0 &       85.936 \\


==> table-data/magic-square-100.tex <==
 1 &      189.957 &    1.0 &     9013.330 &    1.0 \\
 2 &       31.975 &    5.9 &      143.270 &   62.9 \\
 4 &       20.532 &    9.3 &       59.170 &  152.3 \\
 8 &       13.686 &   13.9 &       58.350 &  154.5 \\
12 &        8.677 &   21.9 &       16.860 &  534.6 \\
16 &        8.387 &   22.6 &       17.830 &  505.5 \\


==> table-data/magic-square-avg.tex <==
 30 &        0.855 &    2.2 &    3.3 &    4.4 &    5.9 &    6.9 &        0.125 \\
 40 &        2.496 &    2.0 &    3.6 &    5.7 &    6.1 &    7.4 &        0.335 \\
 50 &        3.903 &    1.8 &    2.5 &    3.8 &    5.2 &    5.6 &        0.702 \\
 60 &        9.834 &    2.2 &    3.8 &    5.6 &    7.2 &    6.8 &        1.441 \\
 70 &       17.571 &    2.2 &    3.4 &    4.8 &    6.6 &    8.5 &        2.065 \\
 80 &       31.889 &    3.0 &    4.3 &    5.8 &    7.6 &    8.6 &        3.689 \\
 90 &       57.746 &    2.9 &    3.8 &    7.2 &    9.3 &   10.8 &        5.323 \\
100 &      189.957 &    5.9 &    9.3 &   13.9 &   21.9 &   22.6 &        8.387 \\


==> table-data/partit-2600.tex <==
 1 &       29.890 &    1.0 &      105.030 &    1.0 \\
 2 &       17.071 &    1.8 &       84.750 &    1.2 \\
 4 &        7.941 &    3.8 &       29.540 &    3.6 \\
 8 &        4.362 &    6.9 &       14.590 &    7.2 \\
12 &        3.490 &    8.6 &        8.830 &   11.9 \\
16 &        2.716 &   11.0 &        6.160 &   17.1 \\


==> table-data/partit-avg.tex <==
1400 &        6.227 &    2.7 &    3.7 &    6.0 &    7.2 &   11.2 &        0.556 \\
1600 &        7.328 &    1.8 &    3.4 &    6.0 &    7.5 &   10.1 &        0.727 \\
1800 &       11.559 &    2.0 &    3.7 &    6.4 &    9.4 &   10.9 &        1.062 \\
2000 &       13.802 &    1.7 &    3.1 &    6.1 &    9.5 &   10.6 &        1.303 \\
2200 &       18.702 &    2.3 &    3.5 &    6.2 &   10.0 &   10.8 &        1.735 \\
2400 &       21.757 &    2.1 &    3.3 &    5.5 &    7.1 &   10.2 &        2.129 \\
2600 &       29.890 &    1.8 &    3.8 &    6.9 &    8.6 &   11.0 &        2.716 \\


==> table-data/perfect-square-5.tex <==
 1 &      143.436 &    1.0 &      456.470 &    1.0 \\
 2 &       66.775 &    2.1 &      217.330 &    2.1 \\
 4 &       39.180 &    3.7 &      117.410 &    3.9 \\
 8 &       21.481 &    6.7 &       64.330 &    7.1 \\
12 &       13.467 &   10.7 &       47.170 &    9.7 \\
16 &        9.517 &   15.1 &       27.550 &   16.6 \\


==> table-data/perfect-square-avg.tex <==
  1 &       14.844 &    1.9 &    4.9 &    8.1 &   11.3 &   16.6 &        0.894 \\
  2 &       30.395 &    1.5 &    4.4 &    6.7 &   10.0 &   14.4 &        2.105 \\
  3 &       55.973 &    1.6 &    2.9 &    6.5 &   12.7 &   14.1 &        3.963 \\
  4 &       75.915 &    1.8 &    3.0 &    5.4 &    9.3 &   15.4 &        4.933 \\
  5 &      143.436 &    2.1 &    3.7 &    6.7 &   10.7 &   15.1 &        9.517 \\

